Getting it Right: Improving Spatial Consistency in Text-to-Image Models

One of the key shortcomings in current text-to-image (T2I) models is their inability to consistently generate images which faithfully follow the spatial relationships specified in the text prompt. In this paper, we offer a comprehensive investigation of this limitation, while also developing datasets and methods that support algorithmic solutions to improve spatial reasoning in T2I models. We find that spatial relationships are under-represented in the image descriptions found in current vision-language datasets. To alleviate this data bottleneck, we create SPRIGHT, the first spatially focused, large-scale dataset, by re-captioning 6 million images from 4 widely used vision datasets and through a 3-fold evaluation and analysis pipeline, show that SPRIGHT improves the proportion of spatial relationships in existing datasets. We show the efficacy of SPRIGHT data by showing that using only $\sim$0.25% of SPRIGHT results in a 22% improvement in generating spatially accurate images while also improving FID and CMMD scores. We also find that training on images containing a larger number of objects leads to substantial improvements in spatial consistency, including state-of-the-art results on T2I-CompBench with a spatial score of 0.2133, by fine-tuning on <500 images. Through a set of controlled experiments and ablations, we document additional findings that could support future work that seeks to understand factors that affect spatial consistency in text-to-image models.

==> tables/long_short.tex <==
\begin{wraptable}[]{!L}{7.0 cm}
%\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{@{}lcc@{}}
        \toprule
        \multirow{2}{*}{\textbf{Model, Setup}} & \multicolumn{2}{c}{\stackanchor{\textbf{T2I-CompBench }}{\textbf{Spatial Score ($\uparrow$)  }}} \\
         \cmidrule{2-3}
        & Long Captions & Short Captions \\
            \midrule
        SD 1.5, w/o CLIP FT & \hl{0.0910} & 0.0708 \\
        SD 2.1, w/o CLIP FT & \hl{0.1605} & 0.1420 \\
        SD 2.1, w/ CLIP FT & \hl{0.1777} &  0.1230 \\
         \bottomrule
        \end{tabular}
}
\caption{Comparing the T2I-CompBench Spatial Scores between models trained on long and short \textit{spatial} captions. Across multiple setups, we find that longer spatial captions lead to better improvements in spatial consistency.}
\label{tab:long_short}
\end{wraptable}

==> tables/ratio.tex <==
\begin{wraptable}[]{R}{6.0 cm}
%\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{@{}cc@{}}
\toprule
\stackanchor{\textbf{\% of Spatial}}{\textbf{Captions}}  & \stackanchor{\textbf{T2I-CompBench}}{\textbf{Spatial Score}} ($\uparrow$) \\
\midrule
25 & 0.154 \\
\rowcolor{green} 50 & 0.178 \\
75 & 0.161 \\
 100 & 0.140 \\
\bottomrule
\end{tabular}
}
\caption{Comparing the T2I-CompBench Spatial Scores between models trained on varying ratio of spatial captions. Fine-tuning on a ratio of 50\% and 75\% of spatial captions yields optimal  results.}
\label{tab:ratio}
\end{wraptable}
